POD-Attention: Unlocking Full Prefill-Decode Overlap for Faster LLM Inference

Each request in LLM inference goes through two phases: compute-bound prefill and memory-bandwidth-bound decode. To improve GPU utilization, recent systems use hybrid batching that combines the prefill and decode phases of different requests into the same batch. This approach optimizes linear operations but remains inefficient for attention computation because existing attention kernels specialize execution independently for the prefill and decode phases. In this paper, we present POD-Attention - the first GPU kernel that efficiently computes attention for hybrid batches. POD-Attention aims to maximize the utilization of both compute and memory bandwidth by carefully allocating the GPU's resources such that prefill and decode operations happen concurrently on the same multiprocessor. POD-Attention speeds up attention computation by up to $59\%$ (mean $28\%$), enabling higher throughput and lower latency LLM inference compared to the use of independently optimized prefill and decode attention kernels.

==> Sections/3-motivation.tex <==
\section{Motivation}\label{sec:motivation}

We first discuss why many LLM serving systems use hybrid batching today, and then expose a critical inefficiency related to attention computation in such systems. For experiments, we use \llamagqa~\cite{llama-8b-hf} model running on two A100 GPUs with the \sarathiserve scheduler~\cite{sarathiserve2024}.

\begin{figure}[t!]
    \centering
    \ignore{
    \begin{subfigure}[t]{0.8\columnwidth}
        \includegraphics[width=\textwidth]{Figures/background/scheduling_vllm.pdf}
        \caption{vLLM scheduling.}
    \label{fig:background:scheduling_vllm}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\columnwidth}
        \includegraphics[width=\textwidth]{Figures/background/scheduling_hybrid.pdf}
        \caption{Hybrid-batching-based scheduling.}
    \label{fig:background:scheduling_hybrid}
    \end{subfigure}
    }
    \includegraphics[width=0.9\columnwidth]{Figures/background/scheduling.pdf}
    \caption{Impact of scheduling strategies on TTFT and TBT.}
    \label{fig:background:scheduling}
\end{figure}

\subsection{Scheduling trade-offs and hybrid batching}
The computationally distinct nature of prefill and decode leads to a throughput-latency tradeoff in LLM inference~\cite{sarathiserve2024, patel2023splitwise, distserve2024, tetriinfer}, depicted in~\autoref{fig:background:scheduling}. Since decoding is memory-bound, running decodes with a high batch size improves throughput. The decode batch size can be increased by prioritizing prefills over decodes (\autoref{fig:background:scheduling}(a)) --- as done by the original \vllm scheduler~\cite{vllmsosp} . This strategy also enables low TTFT at the expense of very high TBT because the ongoing decodes get stalled when a new prefill is scheduled. \sarathiserve~\cite{sarathiserve2024} proposed \textit{chunked-prefills} coupled with \textit{continuous hybrid batching}~\cite{orca} to optimize for TBT. Chunked-prefills limit the number of prefill tokens to be computed in an iteration, enabling users to control TBT. However, hybrid batching increases TTFT because each prefill chunk experiences interference from co-running decodes. Further, chunking can increase the cost of prefill attention due to repeated KV cache loads, once for each chunk's attention computation~\cite{sarathi2023}. The issue of high TBT has been acknowledged in many real-world deployments. Therefore, many LLM serving systems have adopted chunked-prefills and hybrid batching, including \vllm. \ap{citations}

\autoref{fig:background:hybrid-batching} shows how hybrid batching works in practice. For element-wise operations such as the linear transformations in an FFN, the prefill and decode inputs are multiplied with the same model weights. Hence, the prefill and decode tokens can be easily fused for element-wise operations. However, attention is a sequence-level operation that needs to be computed separately for each request. Since the resource requirements of prefill and decode attention kernels are different, current systems compute them separately using specialized GPU kernels of highly optimized libraries e.g., \flashattn~\cite{flashattention,flashattention2,flash-attention-3} and \flashinfer~\cite{flashinfer}.

\subsection{Optimizing attention computation is important}
\label{sec:motivation:bottleneck}

Optimizing attention computation is important in scenarios of high batch size or high context length (or both) because it consumes a significant fraction of the total runtime in such cases. To corroborate this argument, we conduct experiments with long context requests (16K tokens per request) with \llamagqa using prefill chunk size of 1K tokens. We vary the decode batch size from 8 to 64 and report the mean contribution of prefill and decode attention computation in 16 iterations required to complete the prefill phase of one request. \autoref{fig:motivation:op-breakdown} shows that the contribution of attention computation is about 40\% even at a relatively low batch size of 8, which further increases to as high as 65\% at batch size 64. Therefore, attention latency is the biggest overhead at large batch sizes.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{Figures/background/decode_block.pdf}
    \caption{Computation in a decoder block \simon{What's a decoder block?} for hybrid batches. Linear operations receive prefill and decode input fused whereas attention is computed separately. \simon{What are the $e_1$, etc? What is layer norm, pre-projection, etc? Do you need all of these terms?}}
    \label{fig:background:hybrid-batching}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/motivation-op-breakdown/op_breakdown.pdf}
    \caption{Average contribution of different operations to total runtime with hybrid batching (model: \llamagqa, TP-2). \simon{Can Others be explained a bit better or broken down more? What of it is due to FFN computation?}}
    \label{fig:motivation:op-breakdown}
\end{figure}

\subsection{Opportunity with hybrid batching}
\label{sec:motivation:utilization}

\autoref{fig:banner} shows that prefill and decode attention computations have complementary resource requirements: prefill is compute-bound whereas decode is memory-bandwidth-bound.  Further, both prefill and decode attention kernels can consume a significant fraction of the total time as shown in~\autoref{fig:motivation:op-breakdown}. For example, at batch size 32, both kernels consume roughly equal amount of time ($\approx 25\%$ of the total iteration time each). This example highlights that compute and memory bandwidth are both under-utilized for a significant fraction of runtime in LLM inference. Further, note that these two operations are computed immediately one after the other in every hybrid batch. Therefore, hybrid batching presents an opportunity to improve performance by utilizing the GPU's compute and memory resources simultaneously.

While concurrently computing prefill and decode attention can improve GPU resource utilization, we find that existing solutions are often unable to deliver satisfactory performance. To study this in more detail, we first present a case-study of different techniques that could be used to co-locate prefill and decode attention before discussing the design and implementation of \sysname.
